Combination of Run-1 Exotic Searches in Diboson Final States at the LHC

We perform a statistical combination of the ATLAS and CMS results for the search of a heavy resonance decaying to a pair of vector bosons with the $\sqrt{s}=8$ TeV datasets collected at the LHC. We take into account six searches in hadronic and semileptonic final states carried out by the two collaborations. We consider only public information provided by ATLAS and CMS in the HEPDATA database and in papers published in refereed journals. We interpret the combined results within the context of a few benchmark new physics models, such as models predicting the existence of a {\ensuremath{\mathrm{W^\prime}}\xspace} or a bulk Randall-Sundrum spin--2 resonance, for which we present exclusion limits, significances, $p$-values and best-fit cross sections. A heavy diboson resonance with a production cross section of $\sim$4-5 fb and mass between 1.9 and 2.0 TeV is the exotic scenario most consistent with the experimental results. Models in which a heavy resonance decays preferentially to a WW final state are disfavoured.

==> app-zp.tex <==
\section{$Z' \to WW$ signal}
\label{sec:zp}

We recast the $Z'\to WW$ signal and compare with the $WW$ signal from a bulk KK-graviton hypothesis. 
In both benchmarks the final state bosons are purely longitudinal. Due the different tensor structure in the $XWW$ coupling the $W$-bosons coming from the bulk KK-graviton hypothesis are slightly more central~\cite{eiko}.  
The changes efficiency can be factored as coming from two effects: the basic acceptance and angular dependence of the V-boson tagging. Figure \ref{fig:cutflowsemi} shows the relative difference in efficiency between the mentioned benchmarks in the CMS semi-leptonic channel, both in negligible width. {\bf [EXPLAIN THE  TO-BE-DONE Figure]}

\begin{figure*}[h]\begin{center}
[FIGURE WITH EFFICIENCIES/CUT FLOW]
\caption{\small suggestion to paper \label{fig:cutflowsemi}}
\end{center}\end{figure*}

{\bf [PRACTICAL STRATEGY TO FULLY HADRONIC. AND ATLAS SEMI-LEP]}

==> combo_collaborations.tex <==
\label{sec:PerExperiment}
An additional study was performed to compare from one hand the impact of each collaboration on the global result 
and to validate from the other hand the global combination procedure. 

In a first study all the channels was combined within the experiments within the Bulk Graviton hypothesis characterised 
by a custodial symmetry between $W_LW_L$ and $Z_LZ_L$ final states. %We observe Subsequently the 

%study was performed for the Bulk Graviton model 


\begin{figure*}[h]\begin{center}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_WZ_our_nominal_perExp_fu.pdf}
\includegraphics[width=0.32\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_WZ_our_nominal_perExp_p.pdf}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_WZ_our_nominal_perExp_bf.pdf}\\
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_bulk_our_nominal_perExp_fu.pdf}
\includegraphics[width=0.32\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_bulk_our_nominal_perExp_p.pdf}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_bulk_our_nominal_perExp_bf.pdf}
\caption{\small paper suggestion \label{COMBO_GSTAR}}
\end{center}\end{figure*}


==> perExperiment.tex <==
perExperiment

\begin{figure*}[h]\begin{center}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_WZ_our_nominal_perExp_fu.pdf}
\includegraphics[width=0.32\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_WZ_our_nominal_perExp_p.pdf}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_WZ_our_nominal_perExp_bf.pdf}
\caption{\small paper suggestion \label{COMBO_VV_llJ_JJ}}
\end{center}\end{figure*}

\begin{figure*}[h]\begin{center}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_bulk_our_nominal_perExp_fu.pdf}
\includegraphics[width=0.32\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_bulk_our_nominal_perExp_p.pdf}
\includegraphics[width=0.3\textwidth, angle =0 ]{../limits_comparison/CMS_ATLAS_VV_semiJ_bulk_our_nominal_perExp_bf.pdf}
\caption{\small paper suggestion \label{COMBO_VV_llJ_JJ}}
\end{center}\end{figure*}
